Towards Communication-Efficient and Privacy-Preserving Federated Representation Learning

This paper investigates the feasibility of federated representation learning under the constraints of communication cost and privacy protection. Existing works either conduct annotation-guided local training which requires frequent communication or aggregates the client models via weight averaging which has potential risks of privacy exposure. To tackle the above problems, we first identify that self-supervised contrastive local training is robust against the non-identically distributed data, which provides the feasibility of longer local training and thus reduces the communication cost. Then based on the aforementioned robustness, we propose a novel Federated representation Learning framework with Ensemble Similarity Distillation~(FLESD) that utilizes this robustness. At each round of communication, the server first gathers a fraction of the clients' inferred similarity matrices on a public dataset. Then it ensembles the similarity matrices and train the global model via similarity distillation. We verify the effectiveness of FLESD by a series of empirical experiments and show that, despite stricter constraints, it achieves comparable results under multiple settings on multiple datasets.

==> sections/abs_v0.tex <==
\begin{abstract}
    Despite the effectiveness of the existing frameworks, two real-world challenges remain to be addressed in the field of federated learning: lack of human annotations and system heterogeneity of the clients. This paper investigates the feasibility of leveraging the unlabeled client data by the self-supervised learning method. We first study the property of self-supervised local training and find that it's more robust to the non-\iid-ness than the traditional supervised learning paradigm. Then we propose a novel federated self-supervised contrastive learning framework \ours that supports architecture-agnostic local training and communication-efficient global aggregation. At each round of communication, the server first gathers a fraction of the clients' inferred similarity matrices on a public dataset. Then \ours ensembles the similarity matrices and train the aggregated global model via similarity distillation. We verify the effectiveness of our proposed framework by a series of empirical experiments and show that \ours has two main advantages over the existing methods: it handles the model heterogeneity and is more communication-efficient. The code will be released.
\end{abstract}

==> sections/abs_v1.tex <==
\begin{abstract}
This paper investigates the feasibility of learning good representation space with unlabeled client data in the federated scenario. Existing works trivially inherit the supervised federated learning methods, which does not apply to the model heterogeneity and has potential risk of privacy exposure. To tackle the problems above, we first identify that self-supervised contrastive local training is more robust against the non-\iid-ness than the traditional supervised learning paradigm. Then we propose a novel federated self-supervised contrastive learning framework \ours that supports architecture-agnostic local training and communication-efficient global aggregation. At each round of communication, the server first gathers a fraction of the clients' inferred similarity matrices on a public dataset. Then \ours ensembles the similarity matrices and train the global model via similarity distillation. We verify the effectiveness of our proposed framework by a series of empirical experiments and show that \ours has three main advantages over the existing methods: it handles the model heterogeneity, is less prone to privacy leak, and is more communication-efficient. We will release the code of this paper in the future.
\end{abstract}

==> sections/heterogeneity.tex <==
%%%%%%%%%%% Application to Heterogeneity systems.
\subsection{\ours on Heterogeneous Systems}
\subsubsection{Model heterogeneity.}
\bigblah \bigblah

\subsubsection{Data heterogeneity.}
\bigblah \bigblah

\subsubsection{Algorithm heterogeneity.}
\bigblah \bigblah

==> sections/intro_v0.tex <==
\section{Introduction}
% Why unsupervised federated learning is important.
Federated Learning (FL) seeks to collaboratively train the model distributed across a large network while keeping the clients' private data unseen from each other~\cite{konecny_federated_2016, zhao2018federated, li2019fedmd, li2020federated, lin2020ensemble, wang2020federated}. In the practical setting of federated learning, two significant challenges are facing the practitioners. Firstly, the clients do not hold labeled data for the supervised federated learning framework in many scenarios, e.g., a mobile phone user may take dozens of photos but cannot join the federated training due to the lack of annotation. Secondly, in a network that comprises various types of clients, the heterogeneity of the devices leads to the heterogeneity of the model architectures, which poses difficulties for the existing weight-averaging-based federated learning frameworks.

To tackle the first challenge, we re-investigate the properties of the popular Self-Supervised Learning~(SSL) framework~\cite{wu2018unsupervised, oord2018representation, tian2019contrastive, chen2020simple, he2020momentum} when applied to FL~\cite{van2020towards, zhang2020federated}. By proof-of-concept experiments conducted on multiple datasets, we observe that the local training of SSL is much more robust to the statistical heterogeinity~(non-\iid-ness) than traditional supervised local learning. This applies especially when the local client holds only one single category of the data. It's favorable in federated learning that a learning algorithm possesses robust local training, since it means that the communication between the server and the clients (or among the clients) can be carried out with a low frequency. 

\begin{figure}[t]
  \centering
  \includegraphics[width=.46\textwidth]{figures/small_diagram.pdf}
  \vspace{-0.5em}
  \caption{Federated Self-Supervised Training diagram.}
  \vspace{-0.4em}
\end{figure}

\begin{figure*}[t]
    \vspace{-0.8em}
    \centering
    \includegraphics[width=1\textwidth]{LaTeX/figures/distribution_cifar10.pdf}
    \vspace{-1.4em}
    \caption{Local training of supervised and self-supervised learning on CIFAR10. The top row visualizes the non-\iid-ness of the data distribution, the radius of each circle represents the  size of the local dataset. The bottom row compares the behavior of supervised and self-supervised local training. The self-supervised framework SimCLR is more robust than the supervised method. For specific statistics, please refer to the supplementary material.}
    \label{fig:distribution}
    \vspace{-.4em}
\end{figure*}

Next, to enable the architecture-agnostic training, we propose a new framework, Federated self-supervised Learning via Ensemble Similarity Distillation~(\ours). After certain epochs of local training, the clients return the similarity matrix inferred on a public dataset to the server at each communication round. Then \ours distills the knowledge from the ensembled similarity matrix and distributes the distilled model back to the clients. We demonstrate with thorough empirical experiments that besides yielding a better quality of the representation space, our method is more communication-efficient and can aggregate the knowledge from the heterogeneous clients. Our main contributions are summarized as follows:
\begin{itemize}
    \item We investigate the properties of SSL in the federated scenario and point out that the contrastive learning framework is robust to the statistical heterogeneity.
    \item We design a new federated self-supervised learning algorithm \ours that requires significantly fewer rounds of communications during training and is feasible in the FL system with model heterogeneity.
    \item We conduct extensive case studies on the proposed method \ours, providing insights of its behavior.
\end{itemize}




==> sections/method_old.tex <==
% \section{\ours: Federated self-supervised Learning via Ensemble Similarity Distillation}\label{sec:method}
\section{Methodology: \ours}\label{sec:method}

\subsection{Preliminary: Federated Learning}
Federated learning~(FL) studies how to learn from the data examples distributed across different clients in an extensive network, with all the clients' data privacy protected. Specifically, we seek to minimize the objective:
\begin{align}
    \min_{w} L(w) = \sum_{k=1}^K p_k L_k(w) = \E_k\left[ L_k(w) \right],
\end{align}
where $K$ is the number of the clients, $p_k \leq 0$ representing the importance of the $k$-th client, and $\sum_k p_k = 1$. Due to the intrinsic system and statistical heterogeneity of the varying clients, each client might have different data distribution $\gD_k$ and training objective $l_k$: 
\begin{align}
    L_k(w) \triangleq \E_{x \sim \gD_k} \left[ l_k(x; w) \right].
\end{align}

Unlike traditional distributed training that synchronizes the model at each communication round, federated learning is often faced with the problem of network thrashing and the varying speed of local training~\cite{konecny_federated_2016, zhao2018federated, li2020federated, lin2020ensemble}. It thus cannot be optimized in a communication-frequent manner. A commonly adopted measure is to train each client on the local data for certain epochs and then communicate their results for model aggregation. For simplicity, this paper mainly focuses on training the local model over a unified self-supervised contrastive objective. However, our proposed method is not limited to such application scenario and is applicable when varying local objectives are adopted.

\subsection{Local Self-Supervised Training}
Many federated systems are composed of clients that cannot provide annotations on the local data in the real world. This section describes the existing self-supervised contrastive learning that is adopted as the local training framework for the rest of the paper. Contrastive learning is motivated by the ``multi-view hypothesis'', that the different views of the same data example are likely to represent a close or even the same semantics. Following \citet{oord2018representation}, the objective $\lcl$ trains the model to discern one data point's augmented view (positive) from the rest of the data~(negative):
\begin{align}
    \lcl(f) \triangleq - \E \left[ \log \frac{e^{f(x)^{\top}f(x^+)/\tau}}{e^{f(x)^{\top}f(x^+)/\tau} + \sum_{m=1}^{M_\textnormal{neg}} e^{f(x)^{\top}f(x^-_m) / \tau}}\right], \label{eq:cl}
\end{align}
where $f$ is the encoder network; $x^+$ is the positive view created by a series of data augmentations; $x^-$ is the negative examples independently sampled from the data distribution, and $M_{\textnormal{neg}}$ represents the negative sample size. Typically, in the framework of SimCLR, the negative samples are collected from the other samples within the same batch $M_{\textnormal{neg}}=B-1$. As mentioned above, this training objective is applied across all the local devices, i.e., $l_k = \lcl, \forall k \in \{1, \cdots, K\}$.

In some cases where the non-\iid-ness is extreme, the local data distribution contains only one category of the data, and the negative samples all become ``falsely-negative''. Although it leads to a certain extent of the performance decrease (as verified in \Secref{sec:obs}), the contrastive learning objective remains to be conceptually working: it aims to discern subtle differences among the instances regardless of their semantic labels.

\subsection{Global Ensemble Similarity Distillation}
\subsubsection{Similarity matrix ensemble.} To enable federated training with the system heterogeneity and pose strict constraints on the clients' data privacy, we adopt a publically accessible dataset $\Dpub$ as an anchor for global model aggregation. Specifically, the local knowledge of the clients is extracted through inferring on the public dataset.\yc{not local data or model with privacy exposure risk } 

One way of communication is to send back all the representations yielded by the clients. However, since the clients have misaligned representation spaces after local training, it's more sensible to return the geometric information of their representation space. Therefore we choose to adopt the similarity matrix for global aggregation. 

Specifically, suppose the public dataset $|\Dpub|$=$N$ has $N$ examples and the representation of a data point has dimension $d$. The $k$-th client's representation matrix $R_k$ is defined as $R_k \triangleq f_k(\Dpub) \in \mathbb{R}^{d\times N}$, where $f_k$ is the corresponding encoder network. In self-supervised learning, the final representations are often normalized to the unit hypersphere for better performance~\cite{chen2020simple, he2020momentum, wang2020understanding}. We normalize each representation matrix $R_k$ so that its column vectors are all unit vectors. For simplicity, we regard this as default and make no changes to the notations here. The similarity matrix $M_k$ of $k$-th client is computed as:
\begin{align}
    M_k = R_k^{\top} R_k,
\end{align}
where $M_{k, ij}=M_{k, ji}=\langle R_{k,:i} , R_{k,:j} \rangle$ is the similarity of the $i$-th and $j$-th element of $\Dpub$. At each communication round, \ours collect the similarity matrices from a fraction ($C$) of the clients. We denote the sampled set of similarity matrices as $\gM=\left\{ M_k \right\}$, the cardinality of which is $|\gM|=CK$. 

Now we consider the strategy of combining all the similarity matrices. Typically, one client may focus on a particular knowledge domain while has weak discriminant power on other domain. Trivially averaging the similarity matrices of such clients will introduce too much noise and cause over-smoothing. To tackle this problem, we first use the exponential function to sharpen the similarity matrices and then average them as shown below:
\begin{align}
    \hat{M}_{k,ij} &= \exp\left({M_{k, ij}/\tau_{T}}\right), \forall k,i,j \\
    M &= \frac{1}{|\gM|} \sum_{k=1} \hat{M}_k, \label{eq:sim-ensemble}
\end{align}
where $\tau_T$ is the target temperature regulating the sharpness of the similarity matrix. The smaller $\tau_T$ is, the more spike is the similarity matrix, and the model pays more attention to the representations in a small neighborhood. In practice, $\tau_T$ needs to be smaller than 1 to achieve a good performance, which complies with the experience of \citet{koohpayegani2020compress}. Strictly speaking, the ensembled matrix $M$ yielded by \Eqref{eq:sim-ensemble} no longer remains a similarity matrix due to the change of the value scope, $M_{ij} \in (0, +\infty)$. However, as we will see in the following section, this design is in accordance with the similarity-based knowledge distillation technique and will not be a problem. 

% \begin{algorithm}[t]
%     \SetAlgoLined
%     \SetArgSty{textnormal}
%     \setcounter{AlgoLine}{0}
%     \SetKwFunction{server}{\textsc{Server}}
%     \SetKwFunction{client}{\textsc{ClientUpdate}}
%     \SetKwProg{proc}{Procedure}{}{}

%     %server procedure
%     \proc{\server{}}{
%         $w^{(0)} \leftarrow $ random weight initialization \;
    
%         \For{each communication round $t=1,\cdots, T$}{
%             $S^{(t)} \leftarrow $ random subset ($C$ fraction of the $K$ clients) \;
%             \For{each client $k \in S^{(t)}$ \bf{in parallel}}{
%                 $M^{(t)}_k \leftarrow$ \client{$k$, $w^{(t-1)}$}
%             }
%             $M^{(t)} \leftarrow$ ensemble from  $\gM^{(t)} = \{M^{(t)}_k\}_{k=1}$ \;
            
%             $w^{(t)}_0 \leftarrow w^{(t-1)}$ \;
            
%             \For{each iteration $j=1,\cdots, J$}{
%                 sample a mini-batch of data from $\Dpub$ \;
                 
%                 update $w^{(t)}_j$ by $M^{(t)}$ through \Eqref{eq:esd} \;
%             }
            
%             $w^{(t)} \leftarrow w^{(t)}_J$
%         }
%         \KwRet $w^{(T)}$\;
%     }
    
%     \proc{\client{k, w}}{
%         $w^{(0)}_0 \leftarrow w^{(0)} \leftarrow w$ \;
        
%         \For{each local epoch $e=1,\cdots, E$}{
%             \For{each training round $j=1,\cdots, J$}{
%                 sample a mini-batch of data from $D_k$ \;
                
%                 update to $w^{(e)}_j$ through \Eqref{eq:cl} \;
%             }
            
%             $w^{(e)} \longleftarrow w^{(t)}_J$
%         }
%         $M_k \longleftarrow$ similarity inference on $\Dpub$ with $w^{(E)}$ \;
        
%         \KwRet $M_k$\;
%     }
%   \caption{\textbf{F}ederated self-supervised \textbf{L}earning via \textbf{E}nsemble \textbf{S}imilarity \textbf{D}istillation (\textbf{\ours}). }
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%% Main Table %%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\vspace{-.5em}
\begin{center}
\tablestyle{3pt}{1.25}
\begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
& \multirow{3}{*}{$T$} &\multicolumn{12}{c|}{Linear Probing Acc.} 
& \multicolumn{3}{c}{Transfer Acc.} \\

 & &
 \multicolumn{3}{c|}{\smaller{CIFAR10}} &  
 \multicolumn{3}{c|}{\smaller{CIFAR100}} & 
 \multicolumn{3}{c|}{\smaller{Tiny-ImageNet}} &
 \multicolumn{3}{c|}{\smaller{ImageNet-100}} &
 \multicolumn{3}{c}{\smaller{ImageNet-100 $\rightarrow$ CIFAR100}}
 \\
%  Non-FL    & & 86.3 & & & 55.5 & & \\
 & &
\multicolumn{1}{c}{$\alpha$=100} &
\multicolumn{1}{c}{$\alpha$=1} &
\multicolumn{1}{c|}{$\alpha$=0.01} &
\multicolumn{1}{c}{$\alpha$=100} &
\multicolumn{1}{c}{$\alpha$=1} &
\multicolumn{1}{c|}{$\alpha$=0.01} &
\multicolumn{1}{c}{$\alpha$=100} &
\multicolumn{1}{c}{$\alpha$=1} &
\multicolumn{1}{c|}{$\alpha$=0.01} &
\multicolumn{1}{c}{$\alpha$=100} &
\multicolumn{1}{c}{$\alpha$=1} &
\multicolumn{1}{c|}{$\alpha$=0.01} &
\multicolumn{1}{c}{$\alpha$=100} &
\multicolumn{1}{c}{$\alpha$=1} &
\multicolumn{1}{c}{$\alpha$=0.01} 
\\

\shline
%\multicolumn{1}{l|}{Linear} \\
Non-FL    & $\infty$ & - & 86.3 & - & - & 55.5 & - & - & 42.9 & - & - & 78.0 & - & - & 54.7 & - \\
Min-Local & 0 & 62.9 & 66.5 & 60.4 & 12.4 & 41.8 & 41.2 & 35.0 & 34.7 & 35.3 & 63.7 & 61.5  & 59.0 & 50.2 & 49.0 & \textbf{50.5} \\
\hline
FedAvg    & 10 & 75.6 & 75.2 & \textbf{69.9} & 37.8 & 43.2 & \textbf{44.8} & 37.5 & \textbf{37.3} & \textbf{38.4} & \textbf{68.5} & \textbf{69.5} & \textbf{66.6} & \textbf{50.8} & \textbf{50.2} & 49.2 \\
FedProx   & 10 & 71.3 & 72.3 & 67.5 & 33.9 & 39.4 & 40.6 & 25.1 & 26.0 & 26.3 & 46.1 & 44.6 & 43.2 & 33.6 & 34.0 & 34.6 \\
% FedBN   & & & & & & & & & & & & \\
\hline
\ours     & 2 & \textbf{75.8} & \textbf{76.2} & 69.6 & \textbf{39.2} & \textbf{43.8} & 42.2 & \textbf{38.1} & 37.2 & 36.5 & 66.3 & 65.4 & 58.7 & 50.2 & 48.2 & 49.5\\
\ours-cc  & 1 & 73.2 & 74.4 & 66.2 & 18.9 & 42.1 & 41.4 & 36.4 & 36.4 & 36.5 & 63.8 & 64.3 & 60.6 & \textbf{50.8} & 49.7 & 47.5 \\
% \ours-10\%  & & & & & & & & & & & & 
\end{tabular}
\end{center}
\vspace{-0.7em}
\caption{Comparison with Other Federated Baselines. The total epoch of local training is set as constant $E_\text{total}$=$T\times E_\text{local}$=200. 
$T$: communication rounds. 
$\alpha$: value of Dirichlet distribution controlling the non-\iid-ness of the clients' data. Smaller $\alpha$ denotes more serious non-\iid-ness.
\textbf{Non-FL}: upper bound performance trained on the full dataset.
\textbf{Min-Local}: lower bound performance of local training with no global aggregation.
\textbf{\ours-cc}: the degenerate form ``constant communication'' of \ours.
%\textbf{\ours-10\%}: similarity matrix quantization which occupies 10\% of the original band-width.
}
\label{tab:main}
\vspace{-0.5em}
\end{table*}

\subsubsection{Similarity-based distillation.} Unlike traditional knowledge distillation techniques that minimize the cross-entropy between the teacher and student networks' softened class probabilities~\cite{hinton2015distilling, lin2020ensemble}, similarity-based distillation aims to train a student network that mimics the way the teacher network distributes a population of the representations in the feature space~\cite{koohpayegani2020compress, fang2021seed}. Our goal is to leverage the ensemble similarity matrix as an off-line teacher network guiding the training of the student network. One trivial approach computes the student network's similarity matrix over $\Dpub$ and minimizes its distance between the ensemble similarity matrix $M$. However, it needs to run through the whole dataset to perform a single update, which is computationally inefficient. 

Suppose a series of anchor images $\{x_{j_1}, \cdots, x_{j_m}\}$ are indexed by $\{j_1, \cdots, j_m\}$ where $m$ is the size of the anchor set. For a given query image $x_i$ and a student network $f_S$, the similarity between $x_i$ and the anchor images is computed as $\{ f_S(x_{j_1})^{\top} f_S(x_i), \cdots, f_S(x_{j_m})^{\top} f_S(x_i) \}$. To note here the each representation $f_S(\cdot)$ is also automatically normalized to the unit-length vector as discussed in \Secref{sec:method}. Furthermore, we can define a probability distribution over the anchor images based on the similarities computed above. For the student network, the probability of the $i$-th query for the $j$-th anchor is:
\begin{align}
     q_{j}^{i}=\frac{\exp \left( f_S(x_{j})^{\top} f_S(x_i) / \tau_S\right)}{\sum_{k=1}^{m} \exp \left( f_S(x_{j_k})^{\top} f_S(x_i) / \tau_S\right)}, 
\end{align}
where $\tau_S$ is the student temperature hyper parameter. We set $\tau_S = \tau_T$ following the convention of ComPress because this restriction assures that the probabilities of the student network and target are roughly same-scaled and have close semantic meaning. Different from ComPress and SEED that have access to the teacher model, we can only perform the distillation on the similarity matrices for the sake of data privacy. The target probability $p^i$ is directly retrieved from the ensembled similarity matrix $M$, where the i-th query's probability over the j-th anchor is computed as:
\begin{align}
     p_{j}^{i}=\frac{M_{ij}}{\sum_{k=1}^{m} M_{ij_k}}.
\end{align}

Finally, we define the global aggregation training objective $L_\textnormal{g}$ as the mean KL-divergence between the probabilities over the anchor images of the target and the student network:
\begin{align}
     L_\textnormal{g}(f_S) \triangleq \frac{1}{|\Dpub|} \sum_{i=1} \operatorname{KL}\left( p^i \| q^i \right).
\end{align}

During the training of ensemble similarity distillation, the student network is constantly updated. Therefore re-computing the representations of the anchor images is required, which brings large computational overhead. To address this problem, we adopt a momentum encoder and a momentum queue to maintain the recently computed representations of the anchor images. The momentum encoder is the slow version of the student network and is updated by exponential moving average~(EMA). At each step, the momentum encoder will first encode the mini-batch of the data and update the momentum queue in a first-in-first-out~(FIFO) manner. We spare the computational cost of forward passing the anchor images and achieve better training efficiency.

==> sections/related.tex <==
\section{Related Work}
\subsection{Statistical-heterogeneous Federated Learning}

    Firstly proposed by \cite{konecny_federated_2016} as a method for jointly 
    training machine learning models across a collection of highly 
    distributed clients while preserving users' privacy, federated learning has become a key research area 
    in distributed machine learning. Vanilla federated learning uses FedAvg \cite{mcmahan2017communication} for weight aggregation among
    clients, which is intuitive but has difficulty in working with non-\iid data, i.e., data with statistical heterogeneity.
   \cite{zhao2018federated} firstly proposed to share a global dataset among clients for additional fine-tuning, so as to alleviate the divergence of 
   local models; \cite{li2020federated} introduces a proximal regularization term in place of the global dataset to limit the local update during local training; 
   \cite{li2021fedbn}  proposed to train a federated model with local batch normalization, 
   but this method has difficulty in dealing with text data due to batch normalization's limitation; \cite{wang2020federated} 
   noticed the effect of permutation invariance of neural network parameters
   and proposed FedMA to match the neurons among local models for better tolerance of data heterogeneity. 
   
   However, the common assumption of the above methods is that each client carries the same architecture of model 
   and performs weight aggregation, 
   while our method can carry out collaborative training among heterogeneous clients; 
   In addition, our method performs well on self-supervised tasks, 
   while the aforementioned methods mainly focus on supervised scenarios.


\subsection{Model-heterogeneous Federated Learning}

    Another focus of attention in federated learning is model heterogeneity. In the original framework, 
    all clients tend to agree on a particular architecture of a global model. It is usually the case when
    the clients are low-capacity end devices. However, when it comes to cross-silo \cite{MAL-083} scenario where each
    client has enough capacity as well as computing power and desires to design their unique local model for particular
    downstream tasks, a FedAvg-like weight aggregation scheme will no longer be practical.
    \cite{smith2018federated} is the first attempt trying to suit multi-task learning framework to handle 
    the statistical challenges of federated learning, including fitting separated but related models;
    \cite{yang2019federated} proposed Federated Transfer Learning (FTL) which can handle vertical-split data (data features
    instead of instances are separated among clients, introduced in \cite{liu2019communication}) and heterogeneous
    model architectures simultaneously via transfer learning tricks; \cite{li2019fedmd} introduced knowledge distillation \cite{hinton2015distilling}
    to federated learning, which allows participants (clients) to independently design their models and
    transfer knowledge through logits aggregation, consensus exchange and local fine-tuning. Based on this, \cite{ye2019student, luo2019knowledge,shen2019customizing}
    further proposed knowledge amalgamation to jointly distill knowledge from multiple heterogeneous teachers to one student and then
    use the amalgamated knowledge to boost teachers, and proposed more solid loss functions for better accuracy. 
    \cite{jiang2019improving,fallah2020personalized} proposed to handle heterogeneity through meta learning by taking local models as different tasks. 
    
    Different from the methods above, which may need homogeneous model backbone \cite{jiang2019improving, smith2018federated}, 
    shared logits \cite{li2019fedmd}, or shared hidden-states \cite{ye2019student,luo2019knowledge,shen2019customizing} as extra restrictions,
    our method decouples the model architecture with the aggregation operation, that is, considering local models as blackboxes and using 
    the similarity matrix of outputs produced by global dataset on different clients for distilling, 
    which provides a more general solution to model-heterogeneous issues.

    \subsection{Self-supervised Learning}

    Also known as unsupervised representation learning, self-supervised learning methods are expected to learn data 
    representations without humans providing labeled data. There are two main types of self-supervised learning methods: 
    generative and discriminative.
    Generative approaches learn representation by generating observable data in input space 
     \cite{hinton2006reducing,kingma2013auto,radford2015unsupervised}; Discriminative approaches learn representation
    through pretext tasks which can make use of intra-data features or inter-data correlations as 
    supervised signal  \cite{gidaris2018unsupervised,pathak2017curiosity}. One of the most popular methods is contrastive learning \cite{oord2018representation,chen2020simple}, which makes use of contrastive loss \cite{hadsell2006dimensionality} 
    to learn the common characteristics of 
    similar instances and distinguishing the differences between non-similar examples.  \cite{wang2020understanding} 
    further improved constrastive loss based on closeness and uniformity. Due to its outstanding performance, 
    contrastive learning has also been widely applied to NLP \cite{devlin2019bert}, video \cite{tian2020contrastive} and graph \cite{jin2020self}, etc.

    There are also some concurrent works that explore self-supervised learning in federated scenario 
     \cite{jin2020towards, van2020towards,zhang2020federated}, 
    or use self-supervised tricks to improve federated learning \cite{li2021modelcontrastive}.  \cite{jin2020towards,van2020towards} provide 
    several baselines for utilizing unlabelled data in federated learning, but without detailed analysis
    on the challenges that federated self-supervised learning may face; \cite{zhang2020federated} proposed FedCA
    to deal with the inconsistency of representation spaces and misalignment of representations, but they didn't 
    solve the problem of model heterogeneity. To the best of our knowledge, we are the first that propose to handle
    statistical heterogeneity and model heterogeneity in federated self-supervised learning scenario simultaneously.








==> sections/related_short.tex <==
\section{Related Work}
\subsection{Federated Learning}

Firstly proposed by \cite{konecny_federated_2016} as a method for jointly 
training machine learning models across distributed clients while preserving users' privacy, federated learning has become a key research area 
in distributed machine learning. One important challenge of federated learning is non-\iid data. 
\cite{zhao2018federated} firstly proposed to share a global dataset among clients for additional fine-tuning, so as to alleviate the divergence of 
local models; \cite{li2020federated} introduces a proximal regularization term in place of the global dataset to limit the local update during local training; 
\cite{li2021fedbn}  proposed to train a federated model with local batch normalization; \cite{wang2020federated} proposed FedMA to deal with permutation invariance of neural network parameters for better tolerance of data heterogeneity. 

Another focus of attention in federated learning is model heterogeneity. 
\cite{smith2018federated} is the first attempt trying to apply multi-task learning framework to aggregate separated but related models;
\cite{yang2019federated} proposed to handle vertical-split data and heterogeneous
model architectures simultaneously via transfer learning tricks; \cite{li2019fedmd} introduced knowledge distillation \cite{hinton2015distilling}
to federated learning, which allows clients to independently design their models and
transfer knowledge through logits aggregation, consensus exchange and local fine-tuning;
\cite{jiang2019improving,fallah2020personalized} proposed to handle heterogeneity through meta learning by taking local models as different tasks. 

Different from the methods above, our method considers local models as blackboxes and uses
the similarity matrices of outputs produced by global dataset on different clients for distilling, 
which provides a more general solution to both non-\iid and model-heterogeneous issues. Besides, our method performs well on self-supervised tasks, 
while the aforementioned methods mainly focus on supervised scenarios.

\subsection{Self-supervised Learning}

Also known as unsupervised representation learning, self-supervised learning methods are expected to learn data 
representations without humans providing labeled data. There are two main types of self-supervised learning methods: 
generative and discriminative, which learns representation through generating observable data in input space 
\cite{hinton2006reducing,kingma2013auto,radford2015unsupervised} or pretext tasks \cite{gidaris2018unsupervised,pathak2017curiosity}, respectively. One of the most popular methods is contrastive learning \cite{oord2018representation,chen2020simple}, which makes use of contrastive loss \cite{hadsell2006dimensionality} 
to learn the common characteristics of 
similar instances and distinguishing the differences between non-similar examples.

There are also some concurrent works that explore self-supervised learning in federated scenario.  \cite{jin2020towards,van2020towards} provide 
several baselines for utilizing unlabelled data in federated learning, but without detailed analysis
on the challenges that federated self-supervised learning may face; \cite{zhang2020federated} proposed FedCA
to deal with the inconsistency of representation spaces and misalignment of representations, but didn't 
solve the problem of model heterogeneity. To the best of our knowledge, we are the first that propose to handle
statistical heterogeneity and model heterogeneity in federated self-supervised learning scenario simultaneously.

